Proving the dimension-shift conjecture

We prove the conjecture made by Bern, Dixon, Dunbar, and Kosower that describes a simple dimension shifting relationship between the one-loop structure of N = 4 MHV amplitudes and all-plus helicity amplitudes in pure Yang-Mills theory. The proof captures all orders in dimensional regularisation using unitarity cuts, by combining massive spinor-helicity with Coulomb-branch supersymmetry. The form of these amplitudes can be given in terms of pentagon and box integrals using a generalised D-dimensional unitarity technique which captures the full amplitude to all multiplicities.

==> packlist.tex <==
\usepackage{amsmath,amssymb}
\usepackage{authblk}
\usepackage{setspace}
%\usepackage{axodraw}
\usepackage{slashed}
%\usepackage{hyperref}
\usepackage{bm}
\usepackage{mathtools}
\usepackage{titlesec}
\usepackage{xcolor}
\usepackage{cite}
%\usepackage{ulem}
%font
\usepackage{nimbusserif}
\usepackage[T1]{fontenc}
%format
%\usepackage[margin=1in]{geometry}
\titleformat{\section}
  {\normalfont\Large\bfseries}{\thesection}{1em}{}[{\color{gray}\titlerule[0.4pt]}]

